PRISM (Polarized Radiation Imaging and Spectroscopy Mission): A White Paper on the Ultimate Polarimetric Spectro-Imaging of the Microwave and Far-Infrared Sky

PRISM (Polarized Radiation Imaging and Spectroscopy Mission) was proposed to ESA in response to the Call for White Papers for the definition of the L2 and L3 Missions in the ESA Science Programme. PRISM would have two instruments: (1) an imager with a 3.5m mirror (cooled to 4K for high performance in the far-infrared---that is, in the Wien part of the CMB blackbody spectrum), and (2) an Fourier Transform Spectrometer (FTS) somewhat like the COBE FIRAS instrument but over three orders of magnitude more sensitive. Highlights of the new science (beyond the obvious target of B-modes from gravity waves generated during inflation) made possible by these two instruments working in tandem include: (1) the ultimate galaxy cluster survey gathering 10e6 clusters extending to large redshift and measuring their peculiar velocities and temperatures (through the kSZ effect and relativistic corrections to the classic y-distortion spectrum, respectively) (2) a detailed investigation into the nature of the cosmic infrared background (CIB) consisting of at present unresolved dusty high-z galaxies, where most of the star formation in the universe took place, (3) searching for distortions from the perfect CMB blackbody spectrum, which will probe a large number of otherwise inaccessible effects (e.g., energy release through decaying dark matter, the primordial power spectrum on very small scales where measurements today are impossible due to erasure from Silk damping and contamination from non-linear cascading of power from larger length scales). These are but a few of the highlights of the new science that will be made possible with PRISM.

==> alma.tex <==
%% Text from Marcella Massardi, (on behalf of the Italian ARC), Jan Brand
% Rosita Paladino, Elisabetta Liuzzo, Arturo Mignano, Viviana Casasola

\mypar{ALMA:}  
 %
The Atacama Large Millimeter Array (ALMA) can play a complementary role to
the\mission\ mission.
Once completed, the ALMA interferometer will operate in the frequency
range 30-1000 GHz, benefitting from the dryness of the Chilean Chajnantor
plateau. Thanks to the overlap in frequency to the mission it will be the
perfect tool to allow follow-up of sources detected by the satellite,
mapping their structure in total intensity, polarization and spectral line
with richness of detail. ALMA large collecting area ($>6500 m^2$), the
wide range of spatial scales that it covers, and the spectral resolution
(with up to 8192 channels with width between 3.8kHz and 2GHz over 8GHz of
maximum total bandwidth) it will map the sky below declination
$\sim+30^\circ$ with subarcmin FOV and resolution up to a few milliarcsec
with sensitivity as good as few tenths of microJy in continuum and few mJy
for spectral lines in $\sim$1s of observing time.
% *** Could add here that CORE will act as a finding telescope 
% of interesting objects for ALMA to follow up
Hence, it can help to characterize the behavior of the small-scale
foregrounds in the submm bands and define suitable subtraction methods. By
surveying small areas down to a sensitivity well below the CoRE++ mission
detection limits it will allow to characterize the contribution of
foregrounds to the noise on the small angular scales both in total
intensity and polarization. ALMA is expected to detect CMB anisotropies at
the arcsecond scale, as well as the secondary effects (SZ,
Vishniak-Ostriker) that could test the inhomogeneous re-ionization and the nature of
dark energy, complementing the findings of the satellite. The detection of
the SZ effect on scales of a few arcsec will allow to map in detail
clusters and proto-clusters, exploiting the larger scale information
obtained by the satellite detections. The combination of the CoRE++ and
the ALMA telescope will provide an unprecedented tool to astrophysical
investigation in the submm and mm band. The precision of the knowledge of
foregrounds behavior will enhance the already excellent satellite
capabilities to investigate the arcmin scales cosmological information.


==> ccat.tex <==
\mypar{CCAT:}


==> cmb_polar_competition.tex <==
Observations of the B-mode component of the CMB polarisation from suborbital platforms are a very active area of the current research. Over the period of the last few years nearly two dozens of concepts of dedicated CMB B-mode experiment have been described in talks and literature with their deployments envisaged for the forthcoming decade. Some of these proposals involve multiple, staged deployments of progressively more advanced and sensitive experimental set-ups. To date two of such experiments, QUIET \citep[][]{quiet} and BICEP \citep[][]{bicep}, have published results of the analyses of their first data sets, setting up upper limits on the B-mode power and r parameter based on the B-mode polarization, $r \simlt 0.7$ (95\% c.l.). There are a few more experiments currently in operation and data of which are analysed including BICEP/Keck~\citep{bicep/keck}, SPTpol~\citep{sptpol}, ABS~\citep{abs}, EBEX~\citep{ebex}, POLARBEAR \citep[][]{polarbear}, and a few more scheduled for the deployment within a year or so, e.g., QUIJOTE~\citep{quijote}, ACTpol~\citep{actpol} and SPIDER~\citep{spider}. These experiments should start producing results within the next few years and, at the end of that period, are expected to have sufficient sensitivity to provide a convincing first detection of the lensing generated B-mode spectrum and start probing primordial B-modes with r on sub $0.1$ level and possibly down to $r \sim 0.05$ (95\% c.l.). A limit on this level can be also expected from Planck around the same time. On the timescale of a decade or so, more advanced versions of these experiments as well as some new ones, including technologically novel proposals such as bolometric interferometer QUBIC~\citep{qubic}, should reach the sensitivities to detect the gravity waves contribution down to sub $r \sim 0.01$ levels and potentially as low as $r \sim 0.007$ (e.g., POLARBEAR-EXT~\citep{polarbear}, PIPER~\citep{piper}, LSPE~\citep{lspe}). The performance of these last experimental set-ups is typically considered as approaching the limits of what one can expect from the suborbital observations.

Consequently, in the light of these forecast the proposed  mission would improve over the most advanced of the considered suborbital experiments by as much as a factor of $\sim 7$, thanks to its nearly full sky coverage and outstanding sensitivity. It would also permit precise measurements of the B-mode spectrum all the way to the largest angular scales, which are inaccessible to any single suborbital experiment. Moreover it will also ensure a level
of control of systematic effects, which is unachievable from the ground or a balloon. Indeed, those are systematic effects,  of instrumental and astrophysical origins, which are expected to play a major
role in determination of the actual performance of the suborbital observations. In contrast a space mission as the one proposed here will possess an exquisite control of the systematic effects due to the combination of benefits of the space environment at L2 and of its advanced hardware design. The overall gains from such a mission will therefore surely exceed the estimates based solely on the statistical considerations quoted earlier.

We note that even if r happens to be large, i.e., $r \simgt 0.01$, so that first hints of such a signal could be potentially seen by some of the most powerful suborbital experiments, even then its precise characterization and scientific exploitation will be nevertheless only possible by a satellite mission.


==> dustpolar.tex <==
The unique combination of spectral and spatial information provided by the 
CoRE++ survey will open a new dimension to our understanding of dust, its 
nature, and its evolution within interstellar space. 

The Galactic interstellar medium is dusty. Large dust grains (size $> 10$~nm) dominate the dust mass. 
Within the diffuse interstellar medium, the grains are cold ($\sim10-20$~K) and emit at far-IR to millimeter wavelengths. 
Dipolar emission from small carbon dust particles is a main emission component, often refered to as the anomalous microwave emission.
Both dust components are relevant to CoRE observations.  

Dust properties (size, temperature, emissivity) are found to vary from one line of sight to another 
within the diffuse interstellar medium and molecular clouds. These observations indicate that dust grains evolve through 
the interstellar medium. They can grow through the formation of refractory or ice mantles,  or 
by coagulation into aggregates in dense and quiescent regions. They can also be destroyed by 
fragmentation and erosion of their mantles under more violent conditions.  The composition of interstellar 
dust reflects the action of interstellar processes, which contribute to break and re-build grains over timescales 
much shorter than the timescale of injection by  stellar ejecta. While there is wide consensus on 
this view at interstellar dust, the processes that drive its evolution in space are still poorly understood (\cite{Draine09}).   
Understanding interstellar dust evolution is a major challenge  in astrophysics
underlying key physical and chemical processes in interstellar space. 

Polarization observations are a new, essentially unexplored, means
to study interstellar dust.  The polarization of dust emission  is related to grain 
properties (size, shape, and magnetic susceptibility) and the efficiency of grain alignment, which depends 
on local physical conditions (gas density, radiation field). Dust evolution modifies 
the optical properties of dust grains as well as the efficiency of the mechanism that tends to 
align their rotational axis along the magnetic field lines.  
The physical processes that couple dust grains and their alignment with local physical conditions 
make the separation of the Galactic and CMB polarization intrinsically difficult. 
These physical couplings break the simplest assumption by which the spectral frequency 
dependence of the Galactic polarization and its angular structure on the sky are separable.  

There are several questions that we need to answer in order
to characterize the spectral dependence of dust polarization and its variations across the sky. 
Which dust components are polarized? 
How does one account for grain alignment, and what is its dependence on local 
physical conditions? Planck data is providing constraints on existing models  but it lacks the spectral coverage
to discriminate between possible solutions. 
The wide spectral coverage and the large number of spectral bands are unique assets of the CoRE++ project 
to answer these questions.  Success in this challenging endeavor  will be key 
to understand fully how dust polarization acts as a tracer of 
the magnetic field structure within interstellar matter and how
to achieve an optimal accuracy in component separation for the detection of B-modes. 


==> erosita.tex <==
At the time when \mission\ flies, the eROSITA X-ray survey will most likely be the only 
deeper all-sky cluster survey available.
20--30 times more sensitive than ROSAT, 
eROSITA has as its principal goal to explore cosmological models using galaxy clusters.  
Current forecasts predict that eRosita will detect of order of $10^5$ galaxy with more than 
100 photon counts, which is sufficient to provide a good detection and in many cases to 
detect the source as extended in X-rays. The main survey provides a good sample of galaxy 
clusters typically out to $z=1$ with some very massive and exceptional clusters at larger 
distance.

The large majority of these clusters will be re-detected by the \mission\ mission and thus 
provide an invaluable inter-calibration of X-ray and SZE cluster cosmology, provide 
determinations of cluster temperatures by combining two detection techniques, and obtain 
independent cluster distances for many thousands of clusters where X-ray temperatures and 
shape parameters can be obtained from the X-ray survey.

Having the detection of $\sim10^6$ clusters with \mission, one can further exploit the 
eROSITA survey data. While the above detections refer to safe detection at high 
signal-to-noise, there should be almost $10^6$ clusters detected at low significance with 
S/N reaching values of about 2 (10 - 15 counts in 50 background counts). Similar to the 
stacking of ROSAT X-ray signals in the ROSAT All-Sky Survey for SDSS detected 
clusters (Rykoff et al. 2008) one can extract valuable X-ray information for a large 
fraction of the new clusters.



==> euclid_erosita.tex <==
\mypar{eROSITA: }
\input erosita.tex

\mypar{EUCLID: }
\input euclid.tex

==> introduction.tex <==
Give here contextual elements: IRAS, WMAP, Planck, Herschel, SPICA, COrE.

==> ir_initiatives.tex <==
Few prior infrared telescopes have performed all-sky surveys in the
same bands covered by \mission.  Akari was the last telescope to perform
such observations, but poor sensitivity and resolution along with
limited data access have hindered the usefulness of the telescope's
data.  Several other prior telescopes (Spitzer, Herschel) as well as
the airborne observatory SOFIA and the future mission SPICA have been
about to observe in the 600-4000 GHz range, but these telescopes only
performed observations of limited areas of the sky and, except for a
few deep fields, have pointed at objects already identified in other
bands.  \mission will be able to perform observations with sensitivities
comparable to Herschel but covering the entire sky in many frequency bands.


==> line_emission.tex <==
In the millimeter and sub-millimeter range explored by the Core++ mission a significant fraction 
of the Galactic emission is associated to molecular rotational line transitions being the most 
important ones those from CO, HCN, HCO$^+$ and C-I as indicated in Table~\ref{tab:low-freq-bands}. 
On the one hand this molecular emission is of great astrophysical interest and in particular the 
CO emission that is used to trace molecular clouds in the Interstellar Medium (ISM) where star 
formation takes place \citep{1970ApJ...161L..43W,1972ApJ...174L..43P}. On the other hand they may 
constitute a significant foreground emission for cosmology at low and intermediate Galactic 
latitudes. The most intense of those lines are the CO 1-0, 2-1 and 3-2 transition lines that have 
been mapped over the full-sky by the Planck satellite\citep{planckcollaboration:2013p2912} 
although with poor resolution and low signal-to-noise. CO emission is expected to be polarized by 
the \citet{Goldreich:1981p3154} mechanism. In the presence of even a very weak field, the 
rotational levels split into magnetic sublevels. With an anisotropic radiation field and a 
subcritical cloud density, the population of the different magnetic sub-levels will be unequal, 
and net linear polarization will result. By contrast to thermal dust polarization, CO molecular 
line polarization can have a direction either perpendicular or parallel to the magnetic field 
direction, depending on the relative angles between the magnetic field, the velocity gradient, and 
the line of sight. CO polarization has been measured up to 1-2 \% 
\citep{Lai:2003p3270,Greaves:1999p3103,Girart:1999p3062} in some particular molecular clouds. To 
first order we expect it to vary on very small angular scales (few arcsec) following the magnetic 
field and velocity gradient and thus to cancel out at larger angular scales. The Core++ mission 
because of its unprecedented large number of detectors within a single channel, its spectral 
redundancy and resolution should allow a detailed mapping of molecular emission superseding 
current Planck measurements \citep{planckcollaboration:2013p2912} that were limited both by the 
relative small number of detectors within an observational channel and the precision to which 
their spectral band passes were known. Molecular line polarization should be a negligible 
foreground emission for cosmological studies.


==> magnetic_field.tex <==
The Galactic ecological system cannot be understood
without knowledge about the strength and structure of its magnetic field.
CoRE++ will make possible to understand this elusive but dynamically important
component of galaxies.  

The magnetic field is dynamically tied to  cosmic rays and  the turbulent interstellar gas.  
These three components have  
comparable energy densities indicating that they are in
continuous interaction and providing feedback to each other. 
The importance of the magnetic field for the energetics of the interstellar medium (ISM),  
star formation, and galaxy evolution is widely  
recognized, but its actual role remains quantitatively debated due to the paucity of data on its 
its correlation with interstellar turbulence and the density structure of the ISM. 
 We detail some of the prime questions that CoRE++  will resolve in a unique way.  \\


\noindent
{\bf (1) What is the impact of the magnetic field on the interstellar medium energetics?}\\

Synchrotron emission is a prime tracer of the galactic magnetic field. 
The synchrotron intensity allows  estimation of the total magnetic field
strength, while its polarization fraction gives information about the field structure on both 
global and local scales.  The CoRE++ sensitivity will be far superior to other missions.
It will provide a major step forward in our ability to study  magnetic
fields in the Milky Way disk  and  halo.  The
very accurate, highly resolved and detailed view at the polarization of synchrotron emission will be free of Faraday rotation.
Faraday rotation causes the synchrotron polarization vector
to turn as it propagates through the 
magneto-ionized medium. This greatly complicates
analyzing synchrotron emission and can lead to depolarization. At COrE frequencies, the
observed polarization angle of the synchrotron emission directly
relates to the direction of the magnetic field at the location of
emission. This gives a diagnostic of the Galactic magnetic field
complementary to ground-based observations at lower frequencies 
subject to significant Faraday rotation. 
The CoRE++ data will be an eminent complement to upcoming Faraday 
tomography measurements at lower frequencies 
with LOFAR, eVLA, ASKAP, and the SKA. 

Fluctuations in the synchrotron flux in intensity and polarization provide insight into magnetic turbulence. 
Several characteristic statistical properties are encoded in these data, for example the magnetic 
energy and helicity spectra as well as the spectrum of the magnetic tension force.
The accuracy of the CoRE data will thus provide a unique opportunity to  
study magneto-hydrodynamical turbulence and dynamo action, which govern magnetic field amplification and
the energetics of the ISM. It will drastically increase the spectral range of accurately probed magneto-hydrodynamical modes. Therefore 
the detection potential for relevant plasma physics processes and their characteristic scales such as turbulent energy 
injection and dissipation will be considerably increased.  \\

\noindent
{\bf (2)  What role does the magnetic field play in the evolution and structuring of interstellar 
matter and the onset of star formation?} \\

The interplay between turbulence and magnetic fields is also key to star formation.  To investigate this question one needs
to study the polarization of the dust emission, which traces the magnetic fields within interstellar clouds.
Dust polarimetry in emission traces the interstellar magnetic field projected on the plane of the sky. It is 
possible to estimate the magnetic field intensity from polarimetric maps by relating the local dispersion of polarization angles 
and the local amplitude of the turbulent gas motions, a method first proposed by \cite{Chandrasekhar53}. 

The CoRE++ survey will provide the combination of sensitivity and angular resolution required 
to map continuously the Galactic magnetic field associated with interstellar matter, 
from the diffuse interstellar medium to molecular clouds where pre-stellar cores are formed.
Herschel  far-infrared observations have provided astronomers new insight into how turbulence stirs up gas in the interstellar medium, giving rise to a filamentary, web-like structure within cold molecular clouds. COrE++ will complement these stunning images in a unique way revealing 
with the magnetic field structure. CoRE++ will also complement our view at the density structure by providing the first all-sky images of key gas lines,
in particular the CII fine structure line at $157\,\mu$m which is a key tracer of cold neutral matter.
No other experiment offers such capabilities. Planck data is providing a first insight on the field structure. The on-going analysis shows
that Planck is sensitivity limited at the smallest angular scales (i.e. the $5'$  angular resolution of the 
Planck 353 GHz polarization maps).  
Balloon-borne experiments such as Polar-BLAST and PILOT and the HAWCPol far-IR camera on SOFIA  will also be sensitivity limited.
Stellar polarization observations will 
continue to florish, but they are intrinsically limited to discrete sets of sight lines. 
Ground based telescopes at sub-mm and millimeter wavelengths, in particular ALMA, will
image at sub-arcminute to sub-arcsecond angular scales  polarization of compact sources with high column densities (pre- and proto-stellar
condensations, proto-planetary disks). These observations will be complementary to the whole sky survey  of extended emission from
the diffuse interstellar medium and molecular clouds that CoRE++ can uniquely do.    


Star formation occurs as a result of the action of gravity, which is 
counteracted by thermal, magnetic and turbulent pressures (\cite{Larson03} and \cite{McKee07}).  
In the diffuse interstellar medium, outside star-forming molecular clouds,  
the kinetic energy from interstellar turbulence and the magnetic energy 
are comparable. Both are much larger than the cloud gravitational binding energy 
and the gas internal energy.  For stars to form, gravity must become, locally at least, the dominant force. 
This occurs where the turbulent energy has dissipated and matter has condensed 
without increasing the magnetic field flux in comparable proportions. When and how frequently does this occur? This question
is key to our physical understanding of what regulates the efficiency of star formation.  
There is a broad consensus that the answer will follow once we have a physical understanding of the 
interplay between interstellar turbulence and the magnetic field structure in interstellar clouds.

The consumption timescale of the molecular gas in the  Milky Way, $\rm \sim 10^9 \, yr$,  is two orders of magnitude 
larger than the dynamical timescale of its giant  molecular clouds (i.e., their cloud crossing time).
The explanation of this observational fact, established in the early 80s with the advent of CO observations, is still a subject of debate.
The first scenario proposed to regulate star formation combines 
long cloud lifetimes and a low star formation efficiency.  According to this scenario, 
molecular clouds are prevented from collapsing on large scales by turbulent and magnetic 
pressures, while star formation is locally controlled by the rate at which material can cross field lines through
ambipolar diffusion.  Observations and numerical simulations are challenging this view (\cite{Ballesteros07}).  
It is increasingly believed, but still debated,
that the bottle-neck to star formation is the formation of magnetically supercritical condensations where the
magnetic pressure is too weak to
counteract gravity. Once formed, these condensations rapidly collapse to form stars.
Star formation would generally be inefficient, because only a small fraction of the matter
reaches this stage within a cloud lifetime.
Under this second paradigm, molecular clouds are 
transient, and dynamically evolving gas concentrations formed out of diffuse 
interstellar matter. This view stresses the importance of imaging 
the field structure over the extended regions 
of molecular clouds and of the diffuse interstellar medium what 
CoRE++  can uniquely do. \\

%Herschel's stunning images of intricate networks of dust and gas filaments within our Milky Way Galaxy provide an illustrated history of star formation. 
%If conditions are right, gravity then takes over and fragments the filaments into compact cores. Deeply embedded inside these cores are protostars, the seeds of new stars that have gently heated their surrounding dust to just a few degrees above absolute zero, revealing their locations to Herschel's heat-sensitive eyes.

%{\bf COrE will provide the missing observations that we need to understand 
%how the interplay between turbulence and magnetic fields determines the initial conditions for star formation 
%within the diffuse  interstellar medium.}  \\

%Hence, there is a clear scientific need to understand  the interplay between
%turbulence and magnetic fields within the diffuse interstellar medium, which leads to the formation of
%pre-stellar condensations. Without CORE our understanding of the role magnetic field plays 
%in star formation will only be addressed through numerical simulations, without direct validation from observations

\noindent
{\bf (3) What is the impact of the magnetic field on the large-scale 
structure and evolution of the Galaxy?}\\

CoRE is expected to provide important new clues concerning 
the effects of the Galactic magnetic field on larger scales by imaging dust polarization in nearby galaxies.
We know that the magnetic field helps support the interstellar gas 
against its own weight in the Galactic gravitational potential 
and that it confines cosmic rays to the Galactic disk.
In this manner, both the magnetic field and cosmic rays partake 
in the overall hydrostatic balance of the interstellar medium,
causing the gaseous disk to become much thicker.
In turn, the thickening of the disk tends to make it unstable to 
the Parker instability (a type of magnetic Rayleigh-Taylor instability).
As this instability develops, magnetic field lines undulate,
and the interstellar gas slides down along the field lines into the magnetic troughs 
accumulating there.
The whole process, it has been suggested, could give birth to new
molecular cloud complexes and ultimately trigger star formation.

The magnetic field is also believed to play an important role 
in disk-halo interactions, although the exact mechanisms involved 
are still poorly understood and debated.
{\it A priori} one expects the magnetic field to impede mass
exchange between the disk and the halo. 
For instance, the magnetic field tends to contain super-bubbles
and prevent them from venting their gas into the halo.
On the other hand, it has been suggested that the magnetic field
might stabilize infalling clouds and enable them
to reach the disk without being disrupted by their dynamical interaction 
with the hot halo gas. 
To test these various ideas, it is crucial to gain a better observational
knowledge of the Galactic magnetic field, particularly in the halo.
Similarly, a better knowledge of the Galactic magnetic field,
both in the disk and in the halo, will make it possible to place 
stronger constraints on the existing dynamo scenarios.  \\

\subsubsection{COrE sensitivity to polarized synchrotron}

Accurate measurements of the polarized synchrotron radiation provide a unique probe to 
understand the structure of the Galactic magnetic field and to study the energy 
distribution of cosmic rays. The WMAP mission has provided first full-sky sensitive measurements of 
synchrotron-dominated sky emission polarization in the 20-90 GHz frequency range,
%\cite{2007ApJS..170..335P}, 
providing also an estimate of the level of contamination by polarized Galactic emission
outside of the Galactic plane, in regions useful for CMB studies.
The polarization maps expected next year from the {\it Planck} LFI 30 GHz channel 
will improve our understanding of this emission, but, likely, not at the so precise level needed to fully exploit 
the so high sensitivity achieved by COrE++ cosmological channels. 
The observing power of the low frequency channels of COrE 
will be ideal to extract the rich information encoded in the Galactic diffuse 
synchrotron component. Synchrotron radiation is intrinsically highly polarized, up to 
70-75\% in a completely regular field. The observed synchrotron polarization depends on 
the uniformity of the field orientation within the resolution element. The typical 
synchrotron sky temperature at 30 GHz---the lowest-frequency COrE++ channel---is $\sim 100-120 
\mu$K at intermediate Galactic latitudes. Assuming a polarization fraction of $\sim 
60\%$, we predict the typical polarized signals to be of order $\sim 65\mu$K, with 
values depending on the features observed. Significantly higher values may be found in 
the loops and spurs, remnants of old supernova events close to the Galactic plane. At 
high latitudes, away from such local features, the expected degree of polarization 
should be only a few percent, resulting in polarized signals of a few $\mu$K. At 
intermediate latitudes, the polarization will lie somewhere between these two extremes.

The design sensitivity of the COrE++ channels at $\nu < 100$ GHz is approximately 
8$\mu$K at a resolution of one arcmin (and, from 90 to 30 GHz, about 6--17 times better at beam FWHM scales), 
resulting into a polarized signal-to-noise ratio (SNR) of about 85 at 30 GHz, significantly better than that of previous CMB satellites.

\subsubsection{Statistical analysis of Galactic magnetic fields with COrE++}

The accuracy of COrE++ polarization information on Galactic magnetic fields will provide a 
unique opportunity to study magneto-hydrodynamical turbulence and dynamo action in great 
detail within our Galaxy. It would greatly improve the reliability of any polarization 
data on small angular scales of the Milky Way in synchrotron light and thereby increase 
the spectral range of accurately probed magneto-hydrodynamical modes. Therefore the 
detection potential for relevant plasma physical processes and the characteristic 
scales of turbulent energy injection and dissipation would be increased considerably. 
Furthermore, accurate Galactic polarization data will be of eminent value for upcoming 
Faraday tomography measurements with telescopes like LOFAR, eVLA, ASKAP, and especially 
the SKA, which has a comparable timeline as COrE++.

\subsubsection{Faraday rotation free polarization}

The COrE++ 30, 36, 43 and 60 GHz channels will provide a very accurate, highly resolved and 
detailed view on the synchrotron emission of our own galaxy. The polarization data 
permits to study the morphology of Galactic magnetic fields on global and local scales. 
CMB experiments measure at high frequencies and reveal there the original polarization 
structure, which do not suffer from Faraday rotation. {\it Planck} is currently increasing the 
angular resolution of such maps to a level comparable to ground based radio telescopes 
and COrE++ will boost the sensitivity and spectral information.

All ground-based radio-band synchrotron measurements of Galactic magnetic fields to date
were carried out at much lower frequencies. Therefore they exhibit a high level of Faraday rotation and 
depolarization within the Galactic plane, hampering a direct analysis. COrE++, by contrast, will 
unveil the polarization structure with essential no Faraday rotation (see Fig.~\ref{fig:galPol1400MHz}). {\bf This data will 
make possible disentangling depolarization phenomena arising from Faraday 
rotation by the Galactic magnetic field and the superposition of contributions with 
different polarization orientations along the line of sight within the beam.} Having this 
unrotated polarization information with high precision will be of importance for at 
least two scientific research directions:

\begin{itemize}

\item Accurately measured fluctuations in the synchrotron flux in intensity and
polarization provide insight into magnetic turbulence. Several characteristic
statistical properties are encoded in this data, for example the energy
and helicity spectra as well as the spectrum of the magnetic tension force.

\item Such data will allow Faraday rotation tomography measurements of
our galaxy, which will be pursued with upcoming instruments like
LOFAR, eVLA, ASKAP, and especially the SKA. Faraday tomography data
can be expected to reveal further statistical information on Galactic fields,
with very promising potential for detecting signatures of magneto-hydrodynamical
processes.
\end{itemize}

\begin{figure}[t]
 \centering
\includegraphics[bb=0 0 502 320,width=\columnwidth]{Figures/galPol22GHz.png}
% galPol22GHz.png: 1004x620 pixel, 72dpi, 35.42x21.87 cm, bb=0 0 1004 620
 \includegraphics[bb=0 0 589 294,width=\columnwidth]{Figures/galPol1400MHz.png}
 % galPol1400MHz.png: 589x294 pixel, 72dpi, 20.78x10.37 cm, bb=0 0 589 294
 \caption{The WMAP 22.8 GHz all-sky polarized intensity map (upper
panel) and the 1.4 GHz all-sky polarized intensity map (lower panel).
The polarized intensities are shown greyscale coded from 0 to 100 $\mu$K
for 22.8 GHz and from 0 to 570 mK for 1.4 GHz. Galactic Faraday-depolarization structures 
are visible in the lower frequency map. Data from 
\cite{2006A&A...448..411W,2007ApJS..170..335P,2008A&A...484..733T} 
and figures from \cite{2008A&A...477..573S}.
}
 \label{fig:galPol1400MHz}
\end{figure}

\subsubsection{Magnetic spectra}

The statistical properties of Galactic magnetic fields imprint themselves on observables
such as the synchrotron intensity, polarization, and Faraday rotation measure.
Methods to extract this information from observational data already exist and are being 
improved.  Quantities highly relevant for an understanding
of Galactic turbulence and dynamo processes are encoded in polarimetric
data. Examples include:
\begin{itemize}
 \item The {\bf magnetic energy spectrum}, which is imprinted on intensity, polarization spectra and 
cross spectra \cite{1982ApJ...261..310S,1983ApJ...271L..49S,1989AJ.....98..244E,1989AJ.....98..256E}.

 \item The {\bf magnetic helicity spectrum}, which can be measured from polarimetric data in 
combination with extragalactic Faraday data \cite{JunklewitzInThesis,JunklewitzInPrep}. 
Magnetic helicity is a key quantity to understand the inner workings of large-scale 
Galactic dynamos \cite{2009PPCF...51l4043B,2006A&A...448L..33S,2007PPCF...49..447S}.

 \item The {\bf magnetic tension force spectrum}, which is encoded in polarimetry data alone, and is 
powerful in discriminating between different magneto-hydrodynamical scenarios 
\cite{2009MNRAS.398.1970W}.

\end{itemize} 
More physical relevant information might be encoded in the data. The above 
examples are only the quantities that are known today, for which a reconstruction from 
COrE++ data should be possible.

Due to our location within the Galaxy, the angular fluctuations in observables 
correspond to physical magnetic field structures of different sizes. Disentangling these fluctuations 
in order to separate different physical scales such as the turbulent injection scale (see e.g. 
\cite{2008ApJ...680..362H}) or dissipative scales will be challenging. Highly accurate 
polarimetric data, with full-sky coverage and {\bf precise} calibration
will be invaluable for this endeavor. The probing of a large range of 
physical scales simultaneously with high angular resolution
makes it possible to monitor diagnostics
of Galactic turbulence and dynamo theory.

{\bf Statistical analysis of the polarized diffuse 
synchrotron emission from WMAP and from radio surveys disagree.
WMAP finds similar E-mode and B-mode angular power spectra
while those obtained from radio surveys differ significantly 
\cite{2006cmb..confE..16B}. Only more accurate measurements free from 
potential systematic effects can resolve
this discrepancy. COrE++ will provide the necessary data and test the proposed 
theoretical models \cite{2011A&A...526A.145F} at different angular scales to understand if the 
origin of this observational disagreement is explained by residual systematics, data analysis errors, 
or results from subtle astrophysical mechanisms.}

%@INPROCEEDINGS{2006cmb..confE..16B,
%   author = {{Burigana}, C.},
%    title = "{Polarized synchrotron emission}",
%booktitle = {CMB and Physics of the Early Universe},
%     year = 2006,
%   eprint = {arXiv:astro-ph/0607469},
%   adsurl = {http://adsabs.harvard.edu/abs/2006cmb..confE..16B},
%  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
%}

%\bibitem[Burigana(2006)]{2006cmb..confE..16B} Burigana, C.\ 2006, in CMB and 
%Physics of the Early Universe

%
%@ARTICLE{2011A&A...526A.145F,
%   author = {{Fauvet}, L. and {Mac{\'{\i}}as-P{\'e}rez}, J.~F. and {Aumont}, J. and 
%	{D{\'e}sert}, F.~X. and {Jaffe}, T.~R. and {Banday}, A.~J. and 
%	{Tristram}, M. and {Waelkens}, A.~H. and {Santos}, D.},
%    title = "{Joint 3D modelling of the polarized Galactic synchrotron and thermal dust foreground diffuse emission}",
%  journal = {\aap},
%archivePrefix = "arXiv",
%   eprint = {1003.4450},
% primaryClass = "astro-ph.CO",
% keywords = {Galaxy: general, polarization, cosmic background radiation},
%     year = 2011,
%    month = feb,
%   volume = 526,
%    pages = {A145+},
%      doi = {10.1051/0004-6361/201014492},
%   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...526A.145F},
%  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
%}

%\bibitem[Fauvet et al.(2011)]{2011A&A...526A.145F} Fauvet, L., et al.\ 2011, \aap, 526, A145 
 
\begin{figure}
 \centering
 \includegraphics[width=\columnwidth,bb=0 0 1204 888]{Figures/tensionForce_spec.png}
 % tensionForce_spec.png: 1204x888 pixel, 72dpi, 42.47x31.33 cm, bb=0 0 1204 888
 \caption{Tension force spectrum reconstructed from mock polarimetry data using the method of Stokes correlators 
(from \cite{2009MNRAS.398.1970W}). The Gaussian random field was constructed to exhibit the same magnetic energy 
spectrum as the magneto-hydrodynamical simulation, but it has a different fourth-order statistic as measured by the Stokes correlators.}
 \label{fig:tension}
\end{figure}

\subsubsection{Faraday tomography}

Faraday tomography provides three-dimensional information on magnetic 
fields and thereby restores some of the information lost in the line-of-sight projection 
of most astronomical observations. The depth information of a synchrotron emitter is 
encoded in the rate of rotation of its polarization angle as a function of wavelength 
$\lambda$. For different sources at different physical depth, and therefore different 
Faraday depth, this rate differs. Mathematically, the observed polarization as a 
function of wavelength squared is the Fourier transformed polarized emission per Faraday 
depth \cite{1966MNRAS.133...67B}.

An inverse Fourier transformation can therefore reveal the polarization per unit Faraday 
depth \cite{2005A&A...441.1217B}. This technique has already been successfully applied to 
radio data \cite{2006AN....327..545B} and is extremely promising for upcoming radio 
telescopes. However the problem for many of these measurements, especially for long 
wavelength telescopes like LOFAR, is that the full $\lambda^2$-space can not be 
examined. In particular, the negative part of this space cannot be probed by 
any instrument. However information in the full $\lambda^2$-space would be required for 
a direct inversion of the Fourier relation. Therefore inverse methods have to be 
applied which benefit from any available information, in particular close to the 
unaccessible negative $\lambda^2$ range. Thus the information close to $\lambda=0$ as 
will be provided by the COre low frequency channels will be of greatest importance 
for Faraday tomography.

Since the Faraday tomographic data will provide much deeper insight into the details of 
Galactic magnetism than the two dimensional information discussed above, it is obvious 
that the scientific return will be even larger. Accurate all-sky COrE++ data will be 
crucial for the success of this technique for exploring the richness of magnetic phenomena in the Galaxy.



==> other_cmb_missions.tex <==
The \mission\ space mission concept and science objectives combines and extends the science case of several previously proposed next-generation CMB missions.
It is a very wide-scope cosmology mission, proposed for the highest possible scientific return while being targetted mainly at a few key objectives: the most precise full sky measurement of CMB temperature and polarisation possible, to constrain in the best possible way the physics of the early universe and the interactions of the CMB photons with structures on their path towards us; a very precise measurement of the CMB spectrum, to investigate the global history of the main radiation component of the Universe and its interaction with matter in various forms; a complete census of baryons in early galaxies and in galaxy clusters, to map large scale structures and velocity flows in the entire observable universe; a full sky atlas of all of the emission of galactic components in intensity and polarization, to study the distribution of interstellar matter in our Galaxy and the role of the galactic magnetic field for star formation and in the dynamics of the interstellar medium.



==> othertelescopes.tex <==
Existing (APEX, ASTE, IRAM 30m, LMT) and future (CCAT) ground-based
single-dish submillimtre observatories are not as sensitive in bands above 300 GHz
as \mission\ would be, mainly because of the limitations of
observing through the atmosphere.  Existing sub-millimeter
interferometers (ALMA, CARMA, PdB Interferometer, SMA) are ill-suited
to observing large fields.  Moreover, most interferometers have no
capabilities to detect large-scale structure, and while ALMA will have
additional antennas for mapping large-scale structure, it is severely
difficult to use the antennas to map continuum emission.  

\mission\  will be able to map large-scale continuum emission at higher
sensitivities than ground based single-dish telescopes and can cover
larger areas than is practical for interferometers.  Bright compact
sources found by \mission\ in its all-sky surveys can subsequently be
observed in more detail by interferometers.  Moreover, \mission\ can to
provide maps of large scale continuum emission that can be combined
with interferometric data to produce superior maps than what
interferometers can produce by themselves.



==> pixie.tex <==
In 2011, {\it PIXIE} was proposed as an Explorer-class mission to NASA, with the main science objective to constrain large-scale B-modes ($\ell \lesssim 100$) and improve the {\it COBE}/{\it FIRAS} measurements of the CMB spectrum by more than three orders of magnitude \citep{Kogut2011PIXIE}. {\it PIXIE} so far is the only proposed experiment that plans to measure the CMB spectrum. \mission\ is designed to take another step forward. It will combine high resolution polarimetry with absolute calibration, allowing unprecedented control of systematics and foregrounds. While {\it PIXIE} will be unable to detect the distortion signature of dissipating acoustic modes unless the primordial power spectrum shows significant enhancement at small scales, \mission\ spectrometer is specifically designed to detect this signal. This combination of B-mode polarization and CMB frequency spectrum will provide an invaluable probe of inflationary models. Similarly, \mission\ will observe the cosmological recombination lines, supporting our understanding of the Universe some 400 kyrs after the big bang. 


==> ska.tex <==

\mypar{SKA:}  
% text by C. Burigana & K. Grainge
The synergy between the Square Kilometer Array (SKA) and the CoRE++ mission 
is largely based on the complementarity in frequency coverage. 
SKA will span the radio range from 0.07 GHz up to at least 10 
GHz, while possible extension up about 20 GHz have been and are in consideration. 
The definition of the high frequency tail coverage of SKA phase 1 (from some GHz to $\sim 10-15$ GHz) is in progress, while
the highest frequencies will be achieved around 2025 with the SKA phase 2, being fully operative at the time of COrE++ launch. 
SKA is planned to operate for many decades making possible both follow-up observations sources identified by COrE++ and detailed exploration of
the faintest flux densities range.
On of the most relevant perspective offered by the excellent surface brightness sensitivity 
achieved by the so many SKA antennas in a compact core
is the accurate mapping 
out to their virial radius of the majority of the $\sim 10^{6}$ clusters 
that could be detected almost uniformly across 
the whole sky with CoRE++. 
SKA follow-up observations of the good statistical sample provided by CoRE++ up to low masses and high redshifts
 will allow to study magnetic fields in clusters and dark matter through lensing of background radiosources.
SKA will provide also a precise assessment of number counts of SZ effects expected 
by proto-galactic gas heated at the virial temperature and quasar driven blast-waves, making possible accurate prediction 
of the corresponding fluctuations at multipoles of several thousands, relevant for CORE++.
The extreme SKA sensitivity will probe radiosource counts down to $\sim$ tens or hundreds of nJy, 
thus providing important information for their contribution to the background, an aspect crucial for the scientific exploitation of COrE++
CMB absolute temperature. Furthermore, SKA will allow to study the free-free emission associated to cosmological reionization both looking at 
single sources and in statistical sense, as well as, to address the global integrated signal, so complementing at lower frequencies the 
COrE++ spectrum measures.
The cross-correlation of radiosource data (NVSS) and CMB WMAP maps has bean already probed as a fruitful way to detect the 
integrated Sachs-Wolfe (ISW) signal. In about 1-yr, a SKA survey could reveal more $10^{9}(f_{sky}/0.5)$ HI galaxies in a redshift range 0 < z < 1.5, making  
the combination of SKA and the ultimate COrE++ data a powerful (if not the most powerful)
tool for investigating the ISW correlation, thus offering the opportunity to extend our exploitation of the 
statistics of primordial perturbations and of the dark energy dynamics. Also, non-Gaussianity studies will take a large benefit by this kind of data combination.
From the astrophysical point of view, SKA will largely contribute the understanding of galaxy formation and evolution, including AGN feedback, and to the recovery of the
star formation history, complementing with the radio view the COrE++ studies of extragalactic sources and CIB. 
Last but nit least, the exquisite mapping or Galactic radio foreground in both temperature and polarization will greatly contribute to characterize its small scale 
correlation properties and to refine our Galaxy 3D models,
improving quality and physical fundament of the foreground cleaning process necessary for an extremely accurate exploitation of CMB maps. 








